Characterisation of Approximation and (Head) Normalisation for $\lambda\mu$ using Strict Intersection Types

We study the strict type assignment for lambda-mu that is presented in [van Bakel'16]. We define a notion of approximants of lambda-mu-terms, show that it generates a semantics, and that for each typeable term there is an approximant that has the same type. We show that this leads to a characterisation via assignable types for all terms that have a head normal form, and to one for all terms that have a normal form, as well as to one for all terms that are strongly normalisable.

==> eptcsdata.tex <==
\providecommand{\firstpage}{20}
\providecommand{\publicationstatus}{N. Kobayashi (Ed.): Eighth Workshop\\
on Intersection Types and Related Systems (ITRS 2016).\\
EPTCS 242, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.242.4}{10.4204/EPTCS.242.4}}

